X-Align: Cross-Modal Cross-View Alignment for Bird's-Eye-View Segmentation

Bird's-eye-view (BEV) grid is a common representation for the perception of road components, e.g., drivable area, in autonomous driving. Most existing approaches rely on cameras only to perform segmentation in BEV space, which is fundamentally constrained by the absence of reliable depth information. Latest works leverage both camera and LiDAR modalities, but sub-optimally fuse their features using simple, concatenation-based mechanisms. In this paper, we address these problems by enhancing the alignment of the unimodal features in order to aid feature fusion, as well as enhancing the alignment between the cameras' perspective view (PV) and BEV representations. We propose X-Align, a novel end-to-end cross-modal and cross-view learning framework for BEV segmentation consisting of the following components: (i) a novel Cross-Modal Feature Alignment (X-FA) loss, (ii) an attention-based Cross-Modal Feature Fusion (X-FF) module to align multi-modal BEV features implicitly, and (iii) an auxiliary PV segmentation branch with Cross-View Segmentation Alignment (X-SA) losses to improve the PV-to-BEV transformation. We evaluate our proposed method across two commonly used benchmark datasets, i.e., nuScenes and KITTI-360. Notably, X-Align significantly outperforms the state-of-the-art by 3 absolute mIoU points on nuScenes. We also provide extensive ablation studies to demonstrate the effectiveness of the individual components.

==> include/instructions.tex <==
The ABSTRACT is to be in fully-justified italicized text, at the top
of the left-hand column, below the author and affiliation
information. Use the word ``Abstract'' as the title, in 12-point
Times, boldface type, centered relative to the column, initially
capitalized. The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous WACV abstracts to get a feel for style and length.

\section{Introduction}

Please follow the steps outlined below when submitting your manuscript to
the IEEE Computer Society Press.  This style guide now has several
important modifications (for example, you are no longer warned against the
use of sticky tape to attach your artwork to the paper), so all authors
should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the WACV 2023 web page
(\url{http://wacv2023.thecvf.com/submission/})
for a discussion of the policy on dual submissions.

\subsection{Paper length}
Papers must be no longer than eight pages, not including references.
Any pages in excess of eight pages must contain ONLY references ---
no text, figures, acknowledgements, tables, etc.

{\bf There will be no extra page charges for WACV 2023.}

Overlength papers will simply not be reviewed.  This includes papers
where the margins and formatting are deemed to have been significantly
altered from those laid down by this style guide.  Note that this
\LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for
supervised revisions of manuscripts.  The reviewing process cannot determine
the suitability of the paper for presentation in eight pages if it is
reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the
version submitted for review.  The ruler is provided in order that
reviewers may comment on particular lines in the paper without
circumlocution.  If you are preparing a document using a non-\LaTeX\
document preparation system, please arrange for an equivalent ruler to
appear on the final output pages.  The presence or absence of the ruler
should not change the appearance of any other content on the page.  The
camera ready copy should not contain a ruler. (\LaTeX\ users may uncomment
the \verb'\wacvfinalcopy' command in the document preamble.)  Reviewers:
note that the ruler measurements do not align well with lines in the paper
--- this turns out to be very difficult to do well when the paper contains
many figures and equations, and, when done, looks ugly.  Just use fractional
references (e.g.\ this line is $087.5$), although in most cases one would
expect that the approximate location will be adequate.

\subsection{Mathematics}

Please number all of your sections and displayed equations.  It is
important for readers to be able to refer to any particular equation.  Just
because you didn't refer to it in the text doesn't mean some future reader
might not need to refer to it.  It is cumbersome to have to use
circumlocutions like ``the equation second from the top of page 3 column
1''.  (Note that the ruler will not be present in the final copy, so is not
an alternative to equation numbers).  All authors will benefit from reading
Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.


\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind
review.  Blind review does not mean that one must remove
citations to one's own work---in fact it is often impossible to
review a paper unless the previous citations are known and
available.

Blind review means that you do not use the words ``my'' or ``our''
when citing previous work.  In addition, in means you are extremely careful if you
share URLs to source code, github repositories, project websites,
datasets, etc. The URL or other information (e.g. your github user ID)
may identify you and would violate the anonymization policy.


For example, saying ``this builds on the work of Lucy Smith [1]'' does not say
that you are Lucy Smith; it says that you are building on her
work.  If you are Smith and Jones, do not say ``as we show in
[7]'', say ``as Smith and Jones show in [7]'' and at the end of the
paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our
   previous paper [1], and show it to be inferior to all
   previously known methods.  Why the previous paper was
   accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:

\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the
   paper of Smith \etal [1], and show it to be inferior to
   all previously known methods.  Why the previous paper
   was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo
   filter, a fundamental contribution to human knowledge''.
   Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time,
which covers similar or overlapping material, you may need to refer to that
submission in order to explain the differences, just as you would if you
had previously published related work.  In such cases, include the
anonymized parallel submission~\cite{Authors20} as additional material and
cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2020 Submission ID 324,
Supplied as additional material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be
found elsewhere, and refer them to a technical report.  For conference
submissions, the paper must stand on its own, and not {\em require} the
reviewer to go to a techreport for further details.  Thus, you may say in
the body of the paper ``further details may be found
in~\cite{Authors20b}''.  Then submit the techreport as additional material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool which
is widely known to be restricted to a single institution.  For example,
let's say it's 1969, you have solved a key problem on the Apollo lander,
and you believe that the WACV 70 audience would like to hear about your
solution.  The work is a development of your celebrated 1968 paper entitled
``Zero-g frobnication: How being the only people in the world with access to
the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.  Don't write ``We show how to
improve our previous work [Anonymous, 1968].  This time we tested the
algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors. Instead
write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.  This
   system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] didn't
   handle case B properly.  Ours handles it by including
   a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo
   lunar lander, and went all the way to the moon, don't
   you know.  It displayed the following behaviours
   which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention,
reads better than the first version, and does not explicitly name you as
the authors.  A reviewer might think it likely that the new paper was
written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been
contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double blind review policy, you can report results of other challenge participants together with your results in your paper. For your results, however, you should not identify yourself and should not mention your participation in the challenge. Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
\begin{center}
\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
\end{center}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a
sentence-ending space. So \eg is correct, {\em e.g.} is not.  The provided
\verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'',
shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word.)
However, use it only when there are three or more authors.  Thus, the
following is correct: ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...''
because reference~\cite{Alpher03} has just two authors.  If you use the
\verb'\etal' macro provided, then you need not worry about double periods
when used at the end of a sentence as in Alpher \etal.

For this citation style, keep multiple citations in numerical (not
chronological) order, so prefer \cite{Alpher03,Alpher02,Authors20} to
\cite{Alpher02,Alpher03,Authors20}.


\begin{figure*}
\begin{center}
\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\end{center}
   \caption{Example of a short caption, which should be centered.}
\label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}

All text must be in a two-column format. The total allowable width of the
text area is $6\frac78$ inches (17.5 cm) wide by $8\frac78$ inches (22.54
cm) high. Columns are to be $3\frac14$ inches (8.25 cm) wide, with a
$\frac{5}{16}$ inch (0.8 cm) space between them. The main title (on the
first page) should begin 1.0 inch (2.54 cm) from the top edge of the
page. The second and following pages should begin 1.0 inch (2.54 cm) from
the top edge. On all pages, the bottom margin should be 1-1/8 inches (2.86
cm) from the bottom edge of the page for $8.5 \times 11$-inch paper; for A4
paper, approximately 1-5/8 inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area 6-7/8 inches (17.5 cm) wide by 8-7/8 inches (22.54 cm)
high.

Page numbers should be in footer with page numbers, centered and .75
inches from the bottom of the page and make it start at the correct page
number rather than the 9876 in the example.  To do this find the secounter
line (around line 33 in this file) and update the page number as
\begin{verbatim}
\setcounter{page}{123}
\end{verbatim}
where the number 123 is your assigned starting page.

%-------------------------------------------------------------------------
\subsection{Type-style and fonts}

Wherever Times is specified, Times Roman may also be used. If neither is
available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE. Center the title 1-3/8 inches (3.49 cm) from the top edge of
the first page. The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and
adverbs; do not capitalize articles, coordinate conjunctions, or
prepositions (unless the title begins with such a word). Leave two blank
lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type. This information is to
be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT. Type main text in 10-point Times, single-spaced. Do NOT use
double-spacing. All paragraphs should be indented 1 pica (approx. 1/6
inch or 0.422 cm). Make sure your text is fully justified---that is,
flush left and flush right. Please do not place any additional blank
lines between paragraphs.

Figure and table captions should be 9-point Roman type as in
Figures~\ref{fig:onecol} and~\ref{fig:short}.  Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-,
second-, and third-order headings.

FIRST-ORDER HEADINGS. (For example, {\large \bf 1. Introduction})
should be Times 12-point boldface, initially capitalized, flush left,
with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS. (For example, { \bf 1.1. Database elements})
should be Times 11-point boldface, initially capitalized, flush left,
with one blank line before, and one after. If you require a third-order
heading (we discourage it), use 10-point Times, boldface, initially
capitalized, flush left, preceded by one blank line, followed by a period
and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote {This is what a footnote looks like.  It
often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral
observations in
the text (within parentheses, if you prefer, as in this sentence).  If you
wish to use a footnote, place it at the bottom of the column on the page on
which it is referenced. Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times,
single-spaced, at the end of your paper. When referenced in the text,
enclose the citation number in square brackets, for
example~\cite{Authors20}.  Where appropriate, include the name(s) of
editors of referenced books.

\begin{table}
  \begin{center}
    {\small{
\begin{tabular}{llr}
\toprule
Method & Frobnability & Accuracy \\
\midrule
Theirs & Frumpy & 30.2\%\\
Yours & Frobbly & 45.2\%\\
Ours & Makes one's heart Frob & 99.9\%\\
\bottomrule
\end{tabular}
}}
\end{center}
\caption{Results.   Ours are better. If you prefer, you can put table
captions on top of the tables instead of on the bottom.}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.  Please ensure that any point you wish to
make is resolvable in a printed copy of the paper.  Resize fonts in figures
to match the font in the body text, and choose line widths which render
effectively in print.  Many readers (and reviewers), even of an electronic
copy, will choose to print your paper in order to read it.  You cannot
insist that they do otherwise, and therefore must not assume that they can
zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use
\verb+\includegraphics+, and to specify the  figure width as a multiple of
the line width as in the example below
{\small\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.eps}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the WACV 2023 web page 
(\url{http://wacv2023.thecvf.com/submission/})
for a discussion of the use of color in your document.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit
your finished paper. We MUST have this form before your paper can be
published in the proceedings.

Please direct any questions to the production editor in charge of these
proceedings at the IEEE Computer Society Press: 
\url{https://www.computer.org/about/contact}.

==> include/supp_exps.tex <==
%-------------------------------------------------
\section{Varying Backbones}

%-------------------------------------------------
\input{tables/supp_backbones}
%-------------------------------------------------
To verify the generalizability of our X-Align method, we present results for three different encoders, \ie, SWin-T, ConvneXt-T, and ConvneXt-S, in Table~\ref{tab:backbones}. For this ablation study, we choose our \textbf{X-Align}$_{\mathrm{view}}$ variant because this shows that a given model can be improved without adding additional computational complexity during inference. Compared to the current state-of-the-art result from BEVFusion~\cite{liu2022bevfusion}, we can improve their result from 62.7 to 64.1 in terms of mIoU. Similar improvements can be observed for our additionally investigated backbones ConvneXt-T and ConvneXt-S. These results show that our method generalizes well to different backbones without hyperparameter tuning.
%-------------------------------------------------
\section{Adaptability to Noise}

%-------------------------------------------------
\input{tables/supp_noise}
%-------------------------------------------------

Another interesting property of deep neural network-based methods is their susceptibility to input perturbations because it gives insights into their robustness in real environments. Therefore, we add Gaussian noise to the input camera images and observe how the performance degrades in Table~\ref{tab:noise}.  The noise is zero-mean normalized, and $\sigma$ in Table~\ref{tab:noise} is the standard deviation of the Gaussian noise. From the table, we can deduce two main observations: First, the performance of X-Align methods under input perturbations is relatively stable compared to the baseline. We attribute this to the fact that the input camera noise will make the extracted camera feature less reliable. Due to our robust attention-based cross-modal feature fusion (X-FF), the method can still correct the camera features using LiDAR predictions. Our second interesting observation concerns the comparison to the baseline BEVFusion. We observe that our performance loss at a higher noise-variance is much smaller than for BEVFusion, e.g., the performance of our method \textbf{X-Align}$_{\mathrm{all}}$ at $\sigma=0.1$ drops from 65.7 to 59.6. In contrast, BEVFusion drops from 62.7 to 48.9. This shows superior properties of our method in terms of robustness.\par
%-------------------------------------------------
\section{Adverse Weather Conditions}

%-------------------------------------------------
\input{tables/supp_splits}
%-------------------------------------------------

To further investigate our method's robustness, we show results of how our method performs in adverse weather conditions in Table~\ref{tab:splits}. For this experiment, we use the metadata provided by nuScenes, which indicates the weather and light conditions of the recorded scene. With this information, we filter the validation set to obtain two splits containing all images recorded at night and all images recorded during rainy conditions. Our results show consistent improvement in these adverse conditions by \textbf{X-Align}$_{\mathrm{view}}$ as well as \textbf{X-Align}$_{\mathrm{all}}$. This shows that our method improves on comparably easy samples and difficult ones, which is an important property for future deployment of our method.
%-------------------------------------------------
\section{Training Details and Hyperparameter Analysis}

In this subsection, we provide the hyper-parameters and training details for all our experiments in the paper. All our models are trained using Pytorch~\cite{paszke2017automatic} on 4 Nvidia Tesla A100 GPUs.\par

\textbf{nuScenes experiments:} To reproduce the BEVFusion~\cite{liu2022bevfusion} baseline model, we adapt the code provided by their authors\footnote{\href{https://github.com/mit-han-lab/bevfusion}{https://github.com/mit-han-lab/bevfusion}} into the mmdetection3d~\cite{mmdet3d2020} framework. This is because they do not provide training code in the current version. In the camera pipeline, the images are downsampled into a size of $256\times704$ before being passed through a Swin-T~\cite{liu2021swin} or ConvNext~\cite{liu2022convnext} backbone pretrained on ImageNet~\cite{russakovsky2015imagenet}. The intermediate features extracted from the camera are passed through a set of FPN~\cite{lin2017feature} layers to retain the salient low-level encoder features. These are then passed to View-Transformers based on LSS~\cite{philion2020lift}. The baseline is trained using their reported hyper-parameters~\cite{liu2022bevfusion}, with a learning schedule of 20 epochs and a cyclic learning rate, starting for $1e^{-4}$ and performing a single cycle with target ratios $\{10, 1e^{-4}\}$ and a step of $0.4$. For our experiments, we implement our proposed blocks:
\begin{itemize}
\item
\textbf{X-FF Modules}: For the X-FF modules described in Section~\ref{sec:feature_fusion} of the paper, we switch the naive convolutional fuser in the baseline model. To implement the Self-Attention fuser, we tokenize the inputs into patches of size $3\times3$ and a stride of 2. This step is followed by a Multi-Head-Self-Attention block as described in~\cite{vaswani2017attention}, containing 8 heads and an embedding dimension of 256. To implement the Spatial-Channel Attention module, we use the Split-depth Transpose Attention (SDTA) block from EdgeNext~\cite{maaz2022edgenext}.We use an embedding dimension of 256, 2 scales, and 8 heads. We also use DropPath~\cite{larsson2016fractalnet} of $0.1$. A deconvolution block follows the SDTA fusion module to output 256 channels and the fused feature resolution. Finally, to implement the pose-driven deformable convolutional operation, we pass the input pose through a 2-layer MLP network, whose output can is interpolated to the feature size. This pose channel is concatenated with the two input modalities, then passes through a convolutional block to obtain $18$ offset channels, input into a DCNv2~\cite{zhu2019deformable} block of kernel size $3\times3$ The output of the DCNv2 block is our fused feature dimension.
\item
\textbf{X-FA Loss}: As explained in Section~\ref{sec:feature_alignment} of the paper, we use cosine similarity as a loss function to model the X-FA similarity. Using a sparse hyper-parameter search, we set the best value of $\gamma_{2}$ in Equation~(\ref{eq:final_loss}) of the main paper as $-0.002$. We reduce its negative value because we want to increase the cosine similarity.
\item
\textbf{X-SA Module}: As explained in Section~\ref{sec:segmentation_alignment} of the paper, we utilize a perspective decoder to generate 2D perspective view semantic labels. The decoder has two Convolution-BN2D-ReLU sequences with a hidden dimension of $256$ channels, generating semantic probabilities at the output. As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels; we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase.\footnote{\href{https://github.com/Qualcomm-AI-research/InverseForm}{https://github.com/Qualcomm-AI-research/InverseForm}} We pick $\gamma_{3}$ in Equation~(\ref{eq:final_loss}) of the main paper as $0.1$ following a sparse hyper-parameter search. Once we have the 2D perspective features, we share parameters with the LSS Transform from earlier to splat the probability maps to BEV space. We use convolution blocks for channel aggregation at the input and output and interpolate to equalize dimensions. The output is then supervised with BEV GT as shown in Figure~\ref{fig:method_detail1} of the paper. The loss weight $\gamma_4$ is tuned to $0.1$ by observing the total loss value and setting the weight to produce $\sim\! 20\%$ of the total loss. 
\end{itemize}

\textbf{KITTI360 experiments:} To reproduce the PanopticBEV~\cite{gosala22panopticbev} scores, we use the code made public by the authors and their default settings.\footnote{\href{https://github.com/robot-learning-freiburg/PanopticBEV}{https://github.com/robot-learning-freiburg/PanopticBEV}} The model consists of an EfficientDet-d3~\cite{tan2020efficientdet} camera encoder, which encodes multi-resolution features. Next, a multi-scale transformer converts the perspective view to BEV features. This is followed by decoders for both instance and semantics. Finally, their outputs are combined to generate panoptic predictions. The baseline uploaded by the authors reaches a lower value than what was obtained in their paper.  For our experiments with the \textbf{X-SA module}, we added a 2D Perspective decoder to the multi-scale encoded features to predict semantic labels in the perspective view. As KITTI360 contains 2d semantic labels, we use them to supervise this decoder. Then, we reuse the view transformer to map predictions to BEV space. We supervise our X-SA branch with loss weights $\gamma_3$ set at $0.5$ and $\gamma_4$ set at $0.1$, adding them to the total loss of the PanopticBEV baseline.

%As nuScenes~\cite{caesar2020nuscenes} does not contain ground truth segmentation labels; we make use of a state-of-the-art (SOTA) model pre-trained on Cityscapes to generate pseudo labels $\bm{y}^{\mathrm{PV}}$. This is an HRNet-w48~\cite{wang2020deep} checkpoint, trained with the InverseForm~\cite{borse2021inverseform} loss, as made public by the authors in their codebase\footnote{https://github.com/Qualcomm-AI-research/InverseForm}.
%-------------------------------------------------
\section{Qualitative Analysis}

In this Section, we present more sample scenes from nuScenes, as an extension to the one shown in Figure~\ref{fig:qualitative} of the main paper. Each scene consists of 5 parts: a) six surround camera inputs b) LiDAR scan, c) ground-truth BEV segmentation map, d) baseline BEV segmentation, e) BEV segmentation using \textbf{X-Align}$_{\mathrm{view}}$, and d) BEV segmentation \textbf{X-Align}$_{\mathrm{all}}$. For each scenario, we observe that the baseline model prediction is highly erroneous in the region highlighted in \textcolor{green}{green}. We highlight this region of interest in the input views as well. By using our proposed X-SA losses, \textbf{X-Align}$_{\mathrm{view}}$ can already correct substantial errors in the baseline prediction, and the \textbf{X-Align}$_{\mathrm{all}}$ model further improves accuracy.
%-------------------------------------------------
\input{figs/qualitative/supp_qualitative}
%-------------------------------------------------

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tables/nuscenes_det.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lc|cccccc|cc}
        Model & Modality & mAP & NDS \\
        \toprule
        BEVFusion~\cite{liu2022bevfusion} & C &  & \\
        Baseline & C &  & \\
        \textbf{Ours} & C &  & \\
        \bottomrule
    \end{tabular}
    \caption{State-of-the-art comparison on nuScenes det. \textcolor{red}{if we have ablations, then we can add them maybe directly to this Table}}
    \label{tab:nuscenes_det}
\end{table}
